Cross-Lingual Syntactic Transfer with Limited Resources

We describe a simple but effective method for cross-lingual syntactic transfer of dependency parsers, in the scenario where a large amount of translation data is not available. The method makes use of three steps: 1) a method for deriving cross-lingual word clusters, which can then be used in a multilingual parser; 2) a method for transferring lexical information from a target language to source language treebanks; 3) a method for integrating these steps with the density-driven annotation projection method of Rasooli and Collins (2015). Experiments show improvements over the state-of-the-art in several languages used in previous work, in a setting where the only source of translation data is the Bible, a considerably smaller corpus than the Europarl corpus used in previous work. Results using the Europarl corpus as a source of translation data show additional improvements over the results of Rasooli and Collins (2015). We conclude with results on 38 datasets from the Universal Dependencies corpora.

==> code_switch_pseudo.tex <==
\makeatletter
\def\algbackskip{\hskip\dimexpr-\algorithmicindent+\labelsep}
\def\LState{\State \algbackskip}%
\makeatother

\makeatletter
\def\algbackskip{\hskip\dimexpr-\algorithmicindent+\labelsep}
\def\LComment{\Comment \algbackskip}%
\makeatother

\algnewcommand\algorithmicforeach{\textbf{for each}}
\algdef{S}[FOR]{ForEach}[1]{\algorithmicforeach\ #1\ \algorithmicdo}

\begin{figure}[t!]
\hrule width \hsize \kern 1mm \hrule width \hsize height 2pt 
\vspace{0.2cm}
%\noindent\rule{0.5\textwidth}{0.4pt}
\begin{algorithmic}[0]
\small
 \LState {{\bf Inputs: }{ 1) Monolingual texts $\mono_i$ for $i= 1 \ldots (m+1)$; 2) a function $t(w,i,j)$ that translates a word $w \in {\cal L}_i$ to $w' \in {\cal L}_j$; and 3) a parameter $\alpha$ such that $0 < \alpha < 1$.}}
\vspace{0.2cm}
\LState{\bf Algorithm:}
\State ${\cal D} = \{ \}$
\For {$i$ = 1 to $m+1$}
\ForEach {sentence $s \in {\cal D}_i$}
\For {$p = 1$ to $|s|$}
\State Sample $\bar{a} \sim [0,1)$
\If {$\bar{a} \geq \alpha$} \State continue \EndIf
\State Sample $j \sim unif \{1,...,m+1\}\backslash \{i\}$
\State $w' = t (s_p, i, j)$
\If {$w' \neq \nullt$} \State Set $s_p = w'$
\EndIf
\EndFor
\LState${\cal D} = {\cal D} \cup ~\{ s\}$
\EndFor
\EndFor
\State Use the algorithm of \newcite{stratos-collins-hsu:2015:ACL-IJCNLP} on ${\cal D}$
to learn a clustering ${\cal C}$.
\LState {{\bf Output: } The clustering ${\cal C}$.}
\end{algorithmic}

\vspace{0.2cm}

\hrule width \hsize \kern 1mm \hrule width \hsize height 2pt 
\caption{An algorithm for learning a cross-lingual clustering. In
our experiments we used the parameter value $\alpha = 0.3$.}\label{cs_alg2}

\end{figure}


==> count_eq.tex <==
\begin{figure*}[t!]
    \centering
\small
\[
 %\boxed{
\begin{split}
c(w,c)^{\tt new} =\mathbbm{1}{ _{g\stackrel{?}{=}h}}\cdot (1-\alpha)^2  +
\frac{\alpha}{m}[(1-\alpha)   (\sum_{\mathclap{\substack{i=1}}}^{m+1}  ~~ (\sum_{\mathclap{\substack{c'=t(c,g,i)\\i\neq g}}} c(w,c') +
  \sum_{\mathclap{\substack{w'=t(w,h,i)\\i\neq h}}} c(w',c))) 
+  \frac{\alpha}{m}  \sum_{\substack{i,j=1\\i\neq h\\j\neq g}}^{m+1} \sum_{\substack{w',c'\\w'=t(w,h,i)\\c'=t(c,g,j)}}  c(w',c')] 
\end{split}
%}
\]
\caption{The new count value for the co-occurrence count matrix after artificial code-switching. Here $\lang(w)=h$, $\lang(c)=g$ and $\mathbbm{1}{_{...}}$ is the indicator function that is equal to one when the inside condition is true and otherwise zero.}
    \label{fig_new_count}
\end{figure*}


==> discussion.tex <==
\section{Analysis and Discussion}
In this section we provide some discussion and analysis of our results.



\paragraph{Data Requirement Compared to Previous Work}
One of the main points about our model is that all of the mentioned previous work that are compared with our model use either large parallel data such as Europarl or high-coverage bilingual dictionaries. Our model use neither of them. The availability of Bible as a small parallel corpus is a winning factor of our model in terms of data requirements. In practice, we could also use some other available data sets such as Quranic parallel corpus\footnote{\url{http://tanzil.ca/trans/}} for at least 43 languages (some of them with more than one translation), 

%\input{dep_tree}

\paragraph{Effect of Density-Driven Approach}
%As far as we know, this research is the first work that tries to combine the two different parser transfer models and puts them into one model. 
As shown in Table \ref{tab_results1}, for a few languages, we could not achieve any improvement over using Bible projected trees. We believe that the noise from automatic alignments and part of speech errors in the Bible text (because of its domain as a historical text) are two effective reasons for this. We think that more research should be conducted in this trajectory to find much more accurate models that are more robust towards those noise sources.

==> lexicalization_pseudo.tex <==
\begin{figure}[t!]

\hrule width \hsize \kern 1mm \hrule width \hsize height 2pt 
\vspace{0.2cm}
\begin{algorithmic}[0]
\LState {{\bf Inputs: }{ 1) Source treebanks $\tb_i$ for $i=1...m$; 2) function $t(w,i,m+1)$ that translates a word $w \in \lang_i$ to $w' \in \lang_{m+1}$.}}
\vspace{0.1cm}
\LState{\bf Algorithm:}
\For { $i = 1$ to $m$}
\For {sentence $s \in \tb_i$}
\For {$j = 1$ to $|s|$}
\State $w' = t(s_j,i,m+1)$
\State $original\_word(s_j)=s_j$
\State $s_j = w' $ \Comment{{\footnotesize $s_j=\nullt$ iff $ w'=\nullt$}}
\EndFor
\EndFor
\EndFor
\vspace{0.1cm}
\LState {{\bf Outputs: } $\cup_{i=1}^{m}$ modified $\tb_i$}
\end{algorithmic}
\vspace{0.2cm}

\hrule width \hsize \kern 1mm \hrule width \hsize height 2pt 
\caption{Algorithm for lexicalizing the source treebanks with target words.}\label{lx_alg1}
\end{figure}

==> oldintro.tex <==
\section{Introduction} \label{intro}
Creating manually annotated syntactic treebanks is an expensive and time consuming task. Recently there has been a great deal of interest in developing dependency parsers without annotated treebanks: among possible solutions, parser transfer models perform much better than purely unsupervised models~\cite{rasooli-collins:2015:EMNLP}. Transfer models either use translated text and project syntactic dependencies through automatic word alignments to target language sentences  \cite{mcdonald-petrov-hall:2011:EMNLP,ma-xia:2014:P14-1,rasooli-collins:2015:EMNLP}, or directly use treebanks in other languages as training data \cite{tackstrom2013target,yuanregina15,guo2016representation,ammar2016one}.

In this paper we make the following contributions:

\begin{itemize}

\item Cross-lingual representations - brown clusters, embeddings

\item Simple method for lexicalizing treebanks use translation

\end{itemize}

We are interested in the setting where translation data is very limited: specifically Bible data.
Monolingual data is taken from Wikipedia, which is available for many languages.
Integration with the approach of \cite{rasooli-collins:2015:EMNLP} gives ??\%; improvement of ??\%.
Very similar performance to when using Europarl, a much more substantial corpus.

Accurate transfer models that use projection annotations through parallel text rely on a large amount of translation data \cite{rasooli-collins:2015:EMNLP}. On the other hand, direct (non-parallel) models \cite{cohen-das-smith:2011:EMNLP,tackstrom2013target} directly train a parser on a set of source language treebanks. Because of the lexical differences across languages, these models only use delexicalized features and they are usually less accurate than annotation projection models. To provide implicit lexicalization, recent models \cite{yuanregina15,ammar2016one} use multilingual dictionaries or large parallel text to train cross-lingual word representations as their parsing features. The main critique is that if we could obtain parallel text to create representations and dictionaries, we could also apply annotation projection models which are empirically much more accurate than the best direct models. On the other hand, in cases where we deal with  resource-poor languages, we might not have access to multilingual dictionaries or large parallel text. Here is where our motivation for this research comes in.  

This paper designs a transfer model that does not rely on using large parallel text or high-coverage dictionaries. the model only uses the Bible translation data, Wikipedia raw data and treebanks in other languages. Our approach is to extract translation dictionaries from Bible alignments and lexicalize the source treebanks with target words. We also create cross-lingual Brown clustering \cite{brown1992class} and word embeddings from monolingual data by using the translation dictionaries. Brown clustering is used for creating cross-lingual parsing features and the embeddings are used to expand the translation dictionaries.


The main contributions of this paper are: 
\begin{itemize}
      \item We design a model for lexicalizing the source treebanks with the target language words. We create cross-lingual word embeddings with artificial code-switching and employ embedding-based vocabulary expansion  to create artificial translation for those words that have no translation equivalent.
    \item We design an effective way to combine the two transfer models (parallel and non-parallel). We tweak the density-driven model of \cite{rasooli-collins:2015:EMNLP} to simultaneously benefit from the source language treebanks as well as the Bible projected trees for the target language. We show that we can improve the task accuracy and gain results very close to the annotation projection models that make use of much bigger parallel corpora.
\end{itemize}

Our final model obtains a high accuracy comparable to \cite{rasooli-collins:2015:EMNLP} and outperforms \cite{ammar2016one} by 3.8\% absolute LAS and 2.9\% absolute UAS difference. To the best of our knowledge these are the highest accuracies for an approach that makes no use of treebank data for the language of interest and no large parallel corpus. The data and parser from this research will be released along its publication.

The remainder of this paper is as the following:...\todo{fill this in}


==> sup_vs_ours.tex <==
\begin{center}
  \begin{figure*}[ht!]
\scalebox{0.77}{
\centering
 \begin{dependency}[theme = default]
\begin{deptext}
It \& also \& negotiated \& an \& arrangement \& with \& Cable \& News \& Network \& \textcolor{white}{under} \& \textcolor{white}{which} \& \textcolor{white}{CNN} \& would \& agree \& to \& air \& its \& last-minute \& creations \& . \&  $\textcolor{gray}{root}$ \\
\end{deptext}
										
\depedge{3}{1}{\footnotesize nsubj}
\depedge{3}{2}{\footnotesize advmod}
\depedge[edge unit distance=0.9ex]{21}{3}{\footnotesize ROOT}
\depedge{5}{4}{\footnotesize det}
\depedge{3}{5}{\footnotesize dobj}
\depedge{5}{6}{\footnotesize adpmod}
\depedge{9}{7}{\footnotesize compmod}
\depedge{9}{8}{\footnotesize compmod}
\depedge{6}{9}{\footnotesize adpobj}
\depedge[edge unit distance=1.8ex]{14}{10}{\footnotesize rel}
\depedge{10}{11}{\footnotesize adpobj}
\depedge{14}{12}{\footnotesize nsubj}
\depedge{14}{13}{\footnotesize aux}
\depedge[edge unit distance=1.3ex]{5}{14}{\footnotesize rcmod}
\depedge{16}{15}{\footnotesize aux}
\depedge{14}{16}{\footnotesize xcomp}
\depedge{19}{17}{\footnotesize poss}
\depedge{19}{18}{\footnotesize amod}
\depedge{16}{19}{\footnotesize dobj}
\depedge[edge unit distance=0.8ex]{3}{20}{\footnotesize p}

\depedge[edge below,label style={top color=blue!80!pink, bottom color=blue, blue=red, text=white, font=\bfseries},edge unit distance=2ex]{14}{10}{ adpmod}
\depedge[edge below,color=blue,label style={top color=blue!80!pink, bottom color=blue, blue=red, text=white, font=\bfseries}]{12}{11}{ det}
\depedge[edge below,color=blue,label style={top color=blue!80!pink, bottom color=blue, blue=red, text=white, font=\bfseries}]{10}{12}{ adpobj}

\wordgroup[group style={fill=blue!80!pink, draw=blue!40!pink}]{1}{10}{12}{a0}

\end{dependency}
}

     \caption{An example English sentence where the supervised parser could correctly recover the full tree but our model using Europarl has some incorrect dependency predictions (shown at the bottom of the tree).  \label{sup_vs_euro_pic} }
\end{figure*}\end{center}

==> universal_full_tree_table.tex <==
\begin{table}[h]
    \centering
    \begin{tabular}{l|c c}
    \hline
        Lang. & \#sen. & word/sen \\ \hline
        bg & 132 & 12.1 \\
        cs & 193 & 10.4\\
        da & 333 & 12.3\\
        de & 285 & 13.2 \\
        el & 51 & 10.4 \\
        en & 2037 & 18.4 \\
        es & 646 & 14.6 \\
        et & 192 & 9.1 \\
        fa & 25 & 10.6 \\
        fi & 381 & 11.5 \\
        fr & 767 & 16.9\\
        hi & 4  & 9.5 \\
        hr & 122 & 9.2 \\
        hu & 19 & 5.8 \\
        id & 26 & 5.7 \\
        it & 314 & 11.9 \\
        la & 441 & 9.8 \\
        nl & 28 & 7.6 \\
        no & 1049 & 16.4 \\
        pl & 236 & 10.4 \\
        pt & 685 & 15.8 \\
        ro & 120 & 11.8 \\
        ru & 316 & 11.4 \\
        sl & 214 & 11.3 \\
        sv & 733 & 15.6 \\
        tr & 1 & 6 \\ \hline
    \end{tabular}
    \caption{The number of full trees projected from the Bible alignments for the experiments with the Universal dependencies.}
    \label{tab_proj_trees}
\end{table}
